GRIN: GRadient-INformed MoE

Mixture-of-Experts (MoE) models scale more effectively than dense models due to sparse computation through expert routing, selectively activating only a small subset of expert modules. However, sparse computation challenges traditional training practices, as discrete expert routing hinders standard backpropagation and thus gradient-based optimization, which are the cornerstone of deep learning. To better pursue the scaling power of MoE, we introduce GRIN (GRadient-INformed MoE training), which incorporates sparse gradient estimation for expert routing and configures model parallelism to avoid token dropping. Applying GRIN to autoregressive language modeling, we develop a top-2 16$\times$3.8B MoE model. Our model, with only 6.6B activated parameters, outperforms a 7B dense model and matches the performance of a 14B dense model trained on the same data. Extensive evaluations across diverse tasks demonstrate the potential of GRIN to significantly enhance MoE efficacy, achieving 79.4 on MMLU, 83.7 on HellaSwag, 74.4 on HumanEval, and 58.9 on MATH.

==> inputs/5a-inference.tex <==
\subsection{LLM Inference and Serving}

We integrate our \ourmodel into vLLM \citep{kwon2023efficient}, one of the most popular LLM inference and serving libraries. In our analysis, we focus on the H100-80G and A100-80G GPUs and examine the following two scenarios:
\begin{itemize}[leftmargin=*]
\item BF16: As the model size is about 84 GB for BF16, exceeding the memory of a single GPU, we apply tensor parallelism (TP) to distribute the model across two GPUs.
\item FP8: We are particularly interested in single-GPU inference. For the H100, we utilize the existing FP8 support available in vLLM~\footnote{\url{https://github.com/vllm-project/vllm/pull/4343}}. Additionally, we develop FP8 kernels specifically for the A100 to enable efficient one-GPU inference, which can be found in the repository~\footnote{\url{https://github.com/xiaoxiawu-microsoft/vllm/pull/11}}.
\end{itemize}

We benchmarked our results using the repository\footnote{\url{https://github.com/microsoft/DeepSpeedExamples/tree/master/benchmarks/inference/mii}}, with the findings displayed in Figure~\ref{fig:fp16} and Figure~\ref{fig:fp8}. The results provide clear evidence that \ourmodel's serving performance on both H100 and A100 GPUs achieves at least 3$\times$ higher throughput than Mixtral-8$\times$7B given the same first-token latency during the prefilling phase, whether using FP16 or FP8. During the generation phase, \ourmodel demonstrates a 2.5$\times$ reduction in decoding latency and a 3$\times$ increase in inference throughput compared to Mixtral-8$\times$7B. In Appendix~\ref{appendix:inference}, we provide a detailed breakdown of the inference process for \ourmodel, categorizing the operations into dense linear part, sparse expert, multihead attention, and others (including NCCL communication, if applicable).
 % 
%##TO DO experimnet compare M
\begin{figure}
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.45\linewidth]{figure/inference-tp2-h100.pdf}
    \includegraphics[width=0.45\linewidth]{figure/inference-tp2-a100.pdf}
    \caption{FP16: The two left plots represent 2$\times$H100-80g, while the two right plots represent 2$\times$A100-80g. The first and third plots illustrate the pre-filling or prompting phase, and the second and fourth plots depict the decoding or generation phase.}
    \label{fig:fp16}
\end{figure}

\begin{figure}
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.45\linewidth]{figure/inference-tp1-h100.pdf}
        \includegraphics[width=0.45\linewidth]{figure/inference-tp1-a100.pdf}
    \caption{FP8: The two left (right) plots are for 1$\times$H100-80g (1$\times$A100-80g). The description is same as  Figure~\ref{fig:fp16}. }
    \label{fig:fp8}
\end{figure}

%\begin{figure}
%    \centering
%    \vspace{-10pt}
%    \begin{minipage}[b]{0.45\textwidth}
%        \centering
%        \includegraphics[width=1\linewidth]{figure/inference-breakdown-p2048d1024.png}
%        \label{fig:infer_p2048d1024}
%    \end{minipage}
%    \hfill
%    \begin{minipage}[b]{0.45\textwidth}
%        \centering
%        \includegraphics[width=1\linewidth]{figure/inference-breakdown-p4096d1024.png}
%        \label{fig:infer_p2048d1024}
%    \end{minipage}
%\end{figure}

==> inputs/acknowledge.tex <==
% \section*{Acknowledge}

% We would like to thank the engineering team at Microsoft for providing computation infrastructure support.
% Also, we would like to thank
% Abhishek Goswami,
% Alessandro Sordoni,
% Amin Saied,
% Ammar Ahmad Awan,
% Anh Nguyen,
% Benjamin Sorscher,
% Caio César Teodoro Mendes,
% Eric Xihui Lin,
% Gustavo de Rosa,
% Hanxiao Liu,
% Joe Mayer,
% Liliang Ren,
% Marko Radmilac,
% Michael Santacroce,
% Michael Wyatt,
% Mojan Javaheripi,
% Olatunji Ruwase,
% Philipp Witte,
% Russell Hewett,
% Sebastien Bubeck,
% Suriya Gunasekar,
% Xia Song,
% Yadong Lu,
% Yang Liu,
% Yuanzhi Li,
% Yunan Zhang,
% Zichong Li,
% Zhen Zheng,
% \todo{add more (alphabetical order)}
% for their helpful discussions (the name list is organized in the alphabetical order). 



==> table/bbeval.tex <==
\newcommand{\datasetcell}[3]{\makecell{ \large #1  \\  \tiny (#2)    }  }
 
\begin{center}
%\begin{adjustbox}{width=0.95\textwidth,center}

\begin{adjustbox}{width=1\textwidth,center}
\addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{ c||ccccccccc } 
\label{tbl:benchmarks}
&\makecell{Psi\\ \footnotesize 3.8bx16 }& \makecell{Mixtral\\ \footnotesize 8x7b }  & \makecell{Mixtral\\ \footnotesize 8x22b } & \makecell{DeepSeek\\ \footnotesize MoE V2 } &  \makecell{Phi-3\\ \footnotesize 14b  } & \makecell{Mistral\\ \footnotesize 7b } &\makecell{Gemma \\ \footnotesize 7b }&\makecell{Llama-3 \\ \footnotesize 8b }    &  \makecell{GPT-3.5 \\ \footnotesize v1106}  \\
\hline & \\
\datasetcell{MMLU}{5-Shot}{\cite{hendrycks2021measuring} }         & 78.8 & 70.5 & 76.2 & 78.5 & 78.0 & 61.7 & 63.6 & 66.5 & 71.4  \\
\datasetcell{HellaSwag}{5-Shot}{\cite{zellers2019hellaswag} }      & 83.0 & 70.4 & 79.0 & -    & 82.4 & 58.5 & 49.8 & 71.1 & 78.8  \\ 
\datasetcell{ANLI}{7-Shot}{\cite{nie2020adversarial}}              & 58.5 & 55.2 & 65.2 & -    & 55.8 & 47.1 & 48.7 & 57.3 & 58.1  \\
\hline & \\[-1.5ex]
\datasetcell{ GSM-8K}{8-Shot; CoT}{\cite{cobbe2021training} }      & 90.8 & 64.7 & 83.8 & 79.2 & 91.0 & 46.4 & 59.8 & 77.4 & 78.1  \\ 
\datasetcell{Math}{4-Shot; CoT}{\cite{cobbe2021training} }         & 37.3 & 28.5 & 32.8 & 43.6 & 13.1 & 16.7 & 24.5 & 23.3 & 42.6 \\ 
\hline
\datasetcell{ MedQA}{2-Shot}{\cite{jin2020disease} }               & 68.7 & 62.2 & 67.9 & -    & 69.9 & 50.0 & 49.6 & 60.5 & 63.4  \\ 
\datasetcell{ AGIEval}{0-Shot}{\cite{zhong2023agieval} }           & 50.5 & 45.2 & 54.0 & 51.2 & 50.2 & 35.1 & 42.1 & 42.0 & 48.4  \\ 
\datasetcell{ TriviaQA}{5-Shot}{ \cite{joshi2017triviaqa}}         & 73.3 & 82.2 & 84.5 & 79.9 & 73.9 & 75.2 & 72.3 & 67.7 & 85.8 \\ 
\hline & \\[-1.5ex]
\datasetcell{Arc-C}{10-Shot}{\cite{clark2018think} }               & 90.5 & 87.3 & 91.3 & -    & 91.6 & 78.6 & 78.3 & 82.8 & 87.4 \\ 
\datasetcell{Arc-E}{10-Shot}{\cite{clark2018think} }               & 97.7 & 95.6 & 96.9 & -    & 97.7 & 90.6 & 91.4 & 93.4 & 96.3  \\ 
\datasetcell{ PIQA}{5-Shot}{\cite{bisk2019piqa} }                  & 87.3 & 86.0 & 85.0 & -    & 87.9 & 77.7 & 78.1 & 75.7 & 86.6  \\ 
\datasetcell{ SociQA}{5-Shot}{\cite{bisk2019piqa} }                & 78.7 & 75.9 & 78.2 & -    & 80.2 & 74.6 & 65.5 & 73.9 & 68.3  \\ 
\hline & \\[-1.5ex]
\datasetcell{ BigBench-Hard}{3-Shot; CoT}{ }                       & 81.3 & 69.7 & -    & 78.9 & 81.4 & 57.3 & 59.6 & 51.5 & 68.32 \\ 
\datasetcell{WinoGrande}{5-Shot}{\cite{sakaguchi2019winogrande} }  & 79.3 & 62.0 & 75.3 & 84.9 & 81.5 & 54.2 & 55.6 & 65.0 & 68.8  \\ 
\datasetcell{OpenBookQA}{10-Shot}{\cite{mihaylov2018suit} }        & 90.0 & 85.8 & 88.6 & -    & 87.4 & 79.8 & 78.6 & 82.6 & 86.0  \\ 
\datasetcell{BoolQ}{2-Shot}{\cite{clark2019boolq} }                & 83.0 & 77.6 & 82.7 & -    & 86.5 & 72.2 & 66.0 & 80.9 & 79.1  \\ % misantac boolQ incorrectly 77.2 for phi-3-mini on 1st upload, should be 77.6
\datasetcell{CommonSenseQA}{10-Shot}{}                             & -    & 78.1 & 82.0 & -    & 82.8 & 72.6 & 76.2 & 79.0 & 79.6  \\ 
\datasetcell{TruthfulQA}{10-Shot; MC2}{\cite{lin2022truthfulqa} }  & 75.5 & 60.1 & 67.4 & -    & 75.1 & 53.0 & 52.1 & 63.2 & 85.8  \\ 
 
\hline & \\[-1.5ex]
\datasetcell{ HumanEval}{0-Shot}{\cite{chen2021evaluating} }       & 74.3 & 37.8 & 39.6 & 48.8 & 62.2 & 28.0 & 34.1 & 60.4 & 62.2 \\ 
\datasetcell{ MBPP}{3-Shot}{\cite{austin2021program} }             & 79.9 & 60.2 & 70.7 & 66.6 & 75.2 & 50.8 & 51.5 & 67.7 & 77.8  \\ 
\hline & \\[-1.5ex]
Average                                                            & - & 69.8 & & - & -  & 61.2 & 61.7  & 69.4 & 74.3  \\   % phi-small is 
\hline & \\[-1.5ex]
\datasetcell{GPQA}{2-Shot; CoT}{\cite{rein2023gpqa}}               & 36.8 & -  & --& --& --  &-- & -- & & 29.0 \\ 
\datasetcell{MT Bench}{2 round ave.}{\cite{zheng2023judging}}      & 8.62 & -- & & - & 8.91  & --&  --  &--  & 8.35  \\
 
\iffalse
llama-3-70b	
78.2	mmlu
80.0	hella
61.8	anLi
83.7	gsm8k
75.3	medqa
57.3	agieval
85.1	trivia
92.4	arc c
98.0	arc e 
89.3	piqa
78.2	siqa
79.7	bbh
77.7	winogr
92.9	openbookqa
82.7	boolq
84.4	commonsenseqa
55.4	truthqa
40.2	humane
74.9	mbpp
77.22105263	average
\fi
 
 
\end{tabular}
\end{adjustbox}
\end{center}

==> table/bbeval_backup.tex <==
\newcommand{\datasetcell}[3]{\makecell{ \large #1  \\  \tiny (#2) \tiny #3   }  }
 
\begin{center}
%\begin{adjustbox}{width=0.95\textwidth,center}
\begin{adjustbox}{width=1.3\textwidth,center}
\begin{tabular}{ c||cccccccccc } 
\label{tbl:benchmarks}
&\makecell{Psi\\ \footnotesize 3.8bx16 (posttrain) } & \makecell{Phi-3-medium\\ \footnotesize 14b (pretrain) } &  \makecell{Phi-3-medium\\ \footnotesize 14b (posttrain) } & \makecell{Phi-2 \\ \footnotesize 2.7b } & \makecell{Mistral\\ \footnotesize 7b } &\makecell{Gemma \\ \footnotesize 7b }&\makecell{Llama-3-In \\ \footnotesize 8b }  & \makecell{Mixtral\\ \footnotesize 8x7b } & \makecell{Mixtral\\ \footnotesize 8x22b }   &  \makecell{GPT-3.5 \\ \footnotesize version 1106}  \\
\hline & \\[-1.5ex]
 
\datasetcell{MMLU}{5-Shot}{\cite{hendrycks2021measuring} }         & 78.8 & 76.4 & 78.0 & 56.3 & 61.7& 63.6  & 66.5 & 70.5 & 76.2 & 71.4  \\
 
 
\datasetcell{HellaSwag}{5-Shot}{\cite{zellers2019hellaswag} }      & 83.0 & 81.6 &  82.4 & 53.6 & 58.5 & 49.8 & 71.1  & 70.4 & 79.0 & 78.8 \\ 
\datasetcell{ANLI}{7-Shot}{\cite{nie2020adversarial}}              & 58.5 & - &55.8 & 42.5 & 47.1 &  48.7 & 57.3  & 55.2 & 65.2 & 58.1  \\
\hline & \\[-1.5ex]
\datasetcell{ GSM-8K}{8-Shot; CoT}{\cite{cobbe2021training} }      & 90.8 & 85.9  & 91.0& 61.1 & 46.4 &  59.8  & 77.4 & 64.7 & 83.8 & 78.1  \\ 
\hline
\datasetcell{ MedQA}{2-Shot}{\cite{jin2020disease} }               & 68.7 & 63.6 &  69.9 & 40.9 & 50.0  & 49.6  & 60.5 & 62.2 & 67.9 &  63.4  \\ 
\datasetcell{ AGIEval}{0-Shot}{\cite{zhong2023agieval} }           & 50.5 & 46.6  & 50.2 & 29.8 & 35.1  & 42.1  & 42.0 & 45.2 & 54.0 & 48.4  \\ 
\datasetcell{ TriviaQA}{5-Shot}{ \cite{joshi2017triviaqa}}         & 73.3 & 71.9 &73.9 & 45.2 & 75.2  & 72.3 & 67.7   &  82.2 & 84.5 &  85.8 \\ 
\hline & \\[-1.5ex]
\datasetcell{Arc-C}{10-Shot}{\cite{clark2018think} }               & 90.5 & 89.8 & 91.6  & 75.9 & 78.6 & 78.3  & 82.8 & 87.3 & 91.3& 87.4 \\ 
\datasetcell{Arc-E}{10-Shot}{\cite{clark2018think} }               & 97.7 & 97.0 & 97.7& 88.5 & 90.6 & 91.4  & 93.4 & 95.6 & 96.9 & 96.3  \\ 
\datasetcell{ PIQA}{5-Shot}{\cite{bisk2019piqa} }                  & 87.3 &83.0 &87.9 & 60.2 & 77.7 & 78.1  & 75.7 & 86.0 & 85.0 & 86.6  \\ 
\datasetcell{ SociQA}{5-Shot}{\cite{bisk2019piqa} }                & 78.7 & - & 80.2 &68.3 &  74.6 & 65.5 & 73.9  & 75.9 & 78.2 & 68.3  \\ 
\hline & \\[-1.5ex]
 
\datasetcell{ BigBench-Hard}{3-Shot; CoT}{\cite{srivastava2022beyond,suzgun2022challenging} }    
 & 81.33 & - & 81.4 & 59.4 & 57.3  & 59.6  & 51.5 & 69.7 & & 68.32 \\ 
\datasetcell{WinoGrande}{5-Shot}{\cite{sakaguchi2019winogrande} }  & 79.3 & 79.5 & 81.5 & 54.7 & 54.2 & 55.6 & 65.0 & 62.0 & 75.3 & 68.8  \\ 
\datasetcell{OpenBookQA}{10-Shot}{\cite{mihaylov2018suit} }        & 90.0 & 87.8 & 87.4 & 73.6 & 79.8 & 78.6  & 82.6 & 85.8 & 88.6 & 86.0  \\ 
\datasetcell{BoolQ}{2-Shot}{\cite{clark2019boolq} }                & 83.0 & 76.5  & 86.5 & --& 72.2 & 66.0 & 80.9 &77.6 & 82.7 & 79.1  \\ % misantac boolQ incorrectly 77.2 for phi-3-mini on 1st upload, should be 77.6
\datasetcell{CommonSenseQA}{10-Shot}{\cite{talmor2019commonsenseqa} }  & - & 80.9 &82.8 &  69.3 &  72.6 & 76.2 & 79.0 & 78.1 & 82.0 & 79.6  \\ 
\datasetcell{TruthfulQA}{10-Shot; MC2}{\cite{lin2022truthfulqa} }  & 75.5 & 64.7 & 75.1 & --& 53.0 & 52.1  & 63.2 & 60.1 & 67.4 & 85.8  \\ 
 
\hline & \\[-1.5ex]
\datasetcell{ HumanEval}{0-Shot}{\cite{chen2021evaluating} }       & 74.3 & 51.2 & 62.2 & 59.0 & 28.0  & 34.1  & 60.4 & 37.8 & 39.6 & 62.2 \\ 
\datasetcell{ MBPP}{3-Shot}{\cite{austin2021program} }             & 79.9 & 68.1 & 75.2 & 60.6 & 50.8 & 51.5  & 67.7 & 60.2 & 70.7 & 77.8  \\ 
\hline & \\[-1.5ex]
Average                                                            & - & - & - & -- & 61.2 & 61.7  & 69.4 & 69.8 & & 74.3  \\   % phi-small is 
\hline & \\[-1.5ex]
\datasetcell{GPQA}{2-Shot; CoT}{\cite{rein2023gpqa}}               & - & -  & --& --& --&  --  &-- & -- & & 29.0 \\ 
\datasetcell{MT Bench}{2 round ave.}{\cite{zheng2023judging}}      & 8.62 & - & 8.91  & --& --&  --  &--  & -- & & 8.35  \\
 
\iffalse
llama-3-70b	
78.2	mmlu
80.0	hella
61.8	anLi
83.7	gsm8k
75.3	medqa
57.3	agieval
85.1	trivia
92.4	arc c
98.0	arc e 
89.3	piqa
78.2	siqa
79.7	bbh
77.7	winogr
92.9	openbookqa
82.7	boolq
84.4	commonsenseqa
55.4	truthqa
40.2	humane
74.9	mbpp
77.22105263	average
\fi
 
 
\end{tabular}
\end{adjustbox}
\end{center}

==> table/bbeval_backup2.tex <==
\newcommand{\datasetcell}[3]{\makecell{ \large #1  \\  \tiny (#2) \tiny #3   }  }
 
\begin{center}
%\begin{adjustbox}{width=0.95\textwidth,center}
\begin{adjustbox}{width=1.3\textwidth,center}
\begin{tabular}{ c||cccccccccc } 
\label{tbl:benchmarks}
&\makecell{Psi\\ \footnotesize 3.8bx16 (posttrain) } & \makecell{Phi-3-medium\\ \footnotesize 14b (pretrain) } &  \makecell{Phi-3-medium\\ \footnotesize 14b (posttrain) } & \makecell{Phi-2 \\ \footnotesize 2.7b } & \makecell{Mistral\\ \footnotesize 7b } &\makecell{Gemma \\ \footnotesize 7b }&\makecell{Llama-3-In \\ \footnotesize 8b }  & \makecell{Mixtral\\ \footnotesize 8x7b } & \makecell{Mixtral\\ \footnotesize 8x22b }   &  \makecell{GPT-3.5 \\ \footnotesize version 1106}  \\
\hline & \\
%%[-1.5ex]
 
\makecell{\large MMLU \\ \tiny 5-Shot}         & 78.8 & 76.4 & 78.0 & 56.3 & 61.7& 63.6  & 66.5 & 70.5 & 76.2 & 71.4  \\
 
 
\makecell{ \large HellaSwag \\ \tiny 5-Shot}     & 83.0 & 81.6 &  82.4 & 53.6 & 58.5 & 49.8 & 71.1  & 70.4 & 79.0 & 78.8 \\ 
\makecell{\large ANLI\\ \tiny 7-Shot}              & 58.5 & - &55.8 & 42.5 & 47.1 &  48.7 & 57.3  & 55.2 & 65.2 & 58.1  \\
\hline & \\%[-1.5ex]
\makecell{ \large GSM-8K \\ \tiny 8-Shot; CoT}     & 90.8 & 85.9  & 91.0& 61.1 & 46.4 &  59.8  & 77.4 & 64.7 & 83.8 & 78.1  \\ 
\hline
\makecell{ \large MedQA\\ \tiny 2-Shot}             & 68.7 & 63.6 &  69.9 & 40.9 & 50.0  & 49.6  & 60.5 & 62.2 & 67.9 &  63.4  \\ 
\makecell{ \large AGIEval\\ \tiny 0-Shot}           & 50.5 & 46.6  & 50.2 & 29.8 & 35.1  & 42.1  & 42.0 & 45.2 & 54.0 & 48.4  \\ 
\makecell{ \large TriviaQA\\ \tiny 5-Shot}       & 73.3 & 71.9 &73.9 & 45.2 & 75.2  & 72.3 & 67.7   &  82.2 & 84.5 &  85.8 \\ 
\hline & \\%[-1.5ex]
\makecell{\large Arc-C\\ \tiny 10-Shot}               & 90.5 & 89.8 & 91.6  & 75.9 & 78.6 & 78.3  & 82.8 & 87.3 & 91.3& 87.4 \\ 
\makecell{\large Arc-E\\ \tiny 10-Shot}            & 97.7 & 97.0 & 97.7& 88.5 & 90.6 & 91.4  & 93.4 & 95.6 & 96.9 & 96.3  \\ 
\makecell{\large PIQA\\ \tiny 5-Shot}                & 87.3 &83.0 &87.9 & 60.2 & 77.7 & 78.1  & 75.7 & 86.0 & 85.0 & 86.6  \\ 
\makecell{\large SociQA\\ \tiny 5-Shot}               & 78.7 & - & 80.2 &68.3 &  74.6 & 65.5 & 73.9  & 75.9 & 78.2 & 68.3  \\ 
\hline & \\%[-1.5ex]
 
\makecell{\large BigBench-Hard\\ \tiny 3-Shot; CoT}   
 & 81.33 & - & 81.4 & 59.4 & 57.3  & 59.6  & 51.5 & 69.7 & & 68.32 \\ 
\makecell{\large WinoGrande\\ \tiny 5-Shot}  & 79.3 & 79.5 & 81.5 & 54.7 & 54.2 & 55.6 & 65.0 & 62.0 & 75.3 & 68.8  \\ 
\makecell{\large OpenBookQA\\ \tiny 10-Shot}       & 90.0 & 87.8 & 87.4 & 73.6 & 79.8 & 78.6  & 82.6 & 85.8 & 88.6 & 86.0  \\ 
\makecell{\large BoolQ\\ \tiny 2-Shot}           & 83.0 & 76.5  & 86.5 & --& 72.2 & 66.0 & 80.9 &77.6 & 82.7 & 79.1  \\ % misantac boolQ incorrectly 77.2 for phi-3-mini on 1st upload, should be 77.6
\makecell{\large CommonSenseQA\\ \tiny 10-Shot}  & - & 80.9 &82.8 &  69.3 &  72.6 & 76.2 & 79.0 & 78.1 & 82.0 & 79.6  \\ 
\makecell{\large TruthfulQA\\ \tiny 10-Shot; MC2}  & 75.5 & 64.7 & 75.1 & --& 53.0 & 52.1  & 63.2 & 60.1 & 67.4 & 85.8  \\ 
 
\hline & \\%[-1.5ex]
\makecell{\large HumanEval\\ \tiny 0-Shot}      & 74.3 & 51.2 & 62.2 & 59.0 & 28.0  & 34.1  & 60.4 & 37.8 & 39.6 & 62.2 \\ 
\makecell{\large MBPP\\ \tiny 3-Shot}             & 79.9 & 68.1 & 75.2 & 60.6 & 50.8 & 51.5  & 67.7 & 60.2 & 70.7 & 77.8  \\ 
\hline & \\%[-1.5ex]
Average                                                            & - & - & - & -- & 61.2 & 61.7  & 69.4 & 69.8 & & 74.3  \\   % phi-small is 
\hline & \\%[-1.5ex]
\makecell{\large GPQA\\ \tiny 2-Shot; CoT}            & - & -  & --& --& --&  --  &-- & -- & & 29.0 \\ 
\makecell{\large MT Bench\\ \tiny 2 round ave.}     & 8.62 & - & 8.91  & --& --&  --  &--  & -- & & 8.35  \\
 
 
 
\end{tabular}
\end{adjustbox}
\end{center}

==> table/bbeval_lucliu.tex <==
\newcommand{\datasetcell}[3]{\makecell{\large #1  \\[-0.5ex] \tiny (#2)    }  }
 
\begin{table}[t]
\caption{Model Performance on Popular Benchmarks}
\vspace{0.2cm}
\centering
% \caption{Results on the GLUE development set. S refers to Switch and S+S refers to Switch+SparseMixer. AVG is the average score across eight tasks. }
% \resizebox{1.03\linewidth}{!}{
% \hskip-.5cm

\resizebox{1.0\linewidth}{!}{
% \addtolength{\tabcolsep}{-0.3em}
%\hskip-2cm
\begin{tabular}{ c|cccccccccccc } 
% \toprule
& \multicolumn{3}{c}{\large MoE} & \multicolumn{6}{c}{\large Dense} & \multirow{ 2}{*}[-1em]{\makecell{GPT-3.5 \\ \footnotesize v1106 }} & \multirow{ 2}{*}[-1em]{\makecell{GPT-4o \\ \footnotesize 2024}} & \multirow{ 2}{*}[-1em]{\makecell{Gemini \\ \footnotesize 1.5-Flash}}\\
\cmidrule(lr){2-4}
\cmidrule(lr){5-10}
& \ourmodel & \multicolumn{2}{c}{Mixtral} & \multicolumn{2}{c}{Phi3} & Mistral & Gemma & \multicolumn{2}{c}{Llama3} \\
& 16$\times$3.8B & 8$\times$7B & 8$\times$22B  & 14B & 7B & 7B & 7B & 8B & 70B\\ 
% &\makecell{Psi\\ \footnotesize 3.8bx16 }& \makecell{Mixtral\\ \footnotesize 8x7b }  & \makecell{Mixtral\\ \footnotesize 8x22b } & \makecell{DeepSeek\\ \footnotesize V2 } &  \makecell{Phi-3\\ \footnotesize 14b  } &  \makecell{Phi-3\\ \footnotesize 7b  } & \makecell{Mistral\\ \footnotesize 7b } &\makecell{Gemma \\ \footnotesize 7b }&\makecell{Llama-3 \\ \footnotesize 8b }  &\makecell{Llama-3 \\ \footnotesize 70b }&    \\
\midrule 
\datasetcell{MMLU}{5-Shot}{\cite{hendrycks2021measuring} }         & 79.4 & 70.5 & 76.2 & 78.0&75.7 & 61.7 & 63.6 & 66.5 &80.2& 71.4&86.9&79.4  \\[1.5ex]
\datasetcell{HellaSwag}{5-Shot}{\cite{zellers2019hellaswag} }      & 83.7 & 70.4 & 79.0 & 82.4&77.0 & 58.5 & 49.8 & 71.1 &82.6& 78.8&91.7&-  \\[1.5ex]
\datasetcell{ANLI}{7-Shot}{\cite{nie2020adversarial}}              & 60.6 & 55.2 & 65.2 & 55.8&58.1 & 47.1 & 48.7 & 57.3 &68.3& 58.1&75.7&65.6  \\
\midrule 
\datasetcell{ GSM-8K}{8-Shot; CoT}{\cite{cobbe2021training} }      & 90.4 & 64.7 & 83.8 & 91.0&89.6 & 46.4 & 59.8 & 77.4 &93.5& 78.1&93.8&82.4  \\[1.5ex]
% \datasetcell{Math}{0-Shot; CoT}{\cite{cobbe2021training} }         & 58.9 & 11.1 & 41.8 & 46.2&34.6 & 15.0 & 11.4 & 28.2 &51.2& 45.3 &67.8&38.0 \\
\midrule
\datasetcell{ MedQA}{2-Shot}{\cite{jin2020disease} }               & 70.4 & 62.2 & 67.9 & 69.9&65.4 & 50.0 & 49.6 & 60.5 &78.5& 63.4&88.9&-  \\[1.5ex]
\datasetcell{ AGIEval}{0-Shot}{\cite{zhong2023agieval} }           & 48.2 & 45.2 & 54.0 & 50.2&45.1 & 35.1 & 42.1 & 42.0 &56.9& 48.4&37.6&45.2  \\[1.5ex]
\datasetcell{ TriviaQA}{5-Shot}{ \cite{joshi2017triviaqa}}         & 73.9 & 78.5 & 82.2 & 73.9&58.1 & 75.2 & 72.3 & 67.7 &84.5& 85.8&66.0&- \\
\midrule 
\datasetcell{Arc-C}{10-Shot}{\cite{clark2018think} }               & 92.0 & 87.3 & 91.3 & 91.6&90.7 & 78.6 & 78.3 & 82.8 &93.0& 87.4&97.0&88.3 \\[1.5ex]
\datasetcell{Arc-E}{10-Shot}{\cite{clark2018think} }               & 98.0 & 95.6 & 96.9 & 97.7&97.0 & 90.6 & 91.4 & 93.4 &98.2& 96.3&99.0&97.1  \\[1.5ex]
\datasetcell{ PIQA}{5-Shot}{\cite{bisk2019piqa} }                  & 89.0 & 86.0 & 85.0 & 87.9&86.9 & 77.7 & 78.1 & 75.7 &85.3& 86.6&92.9&87.5  \\[1.5ex]
\datasetcell{ SociQA}{5-Shot}{\cite{bisk2019piqa} }                & 79.5 & 75.9 & 78.2 & 80.2&79.2 & 74.6 & 65.5 & 73.9 &81.1& 68.3&81.4&77.8  \\
\midrule 
\datasetcell{ BigBench-Hard}{3-Shot; CoT}{ }                       & 81.4 & 69.7 & 81.8 & 81.4&79.1 & 57.3 & 59.6 & 51.5 & 80.2 & 68.3& 81.2$^*$ &- \\[1.5ex]
\datasetcell{WinoGrande}{5-Shot}{\cite{sakaguchi2019winogrande} }  & 81.4 & 62.0 & 75.3 & 81.5&81.5 & 54.2 & 55.6 & 65.0 &83.3& 68.8&89.3&74.7  \\[1.5ex]
\datasetcell{OpenBookQA}{10-Shot}{\cite{mihaylov2018suit} }        & 89.8 & 85.8 & 88.6 & 87.4&88.0 & 79.8 & 78.6 & 82.6 &91.8& 86.0&95.2&89.0  \\[1.5ex]
\datasetcell{BoolQ}{2-Shot}{\cite{clark2019boolq} }                & 83.4 & 77.6 & 82.7 & 86.5&84.8 & 72.2 & 66.0 & 80.9 &89.1& 79.1&90.6&85.8  \\[1.5ex] 
{\makecell{CommonSenseQA  \\[-0.5ex] \tiny (10-Shot) }}            & 81.8 & 78.1 & 82.0 & 82.8&80.0 & 72.6 & 76.2 & 79.0 &84.4& 79.6&88.5&84.0  \\[1.5ex]
\datasetcell{TruthfulQA}{10-Shot; MC2}{\cite{lin2022truthfulqa} }  & 74.5 & 60.1 & 67.4 & 75.1&70.2 & 53.0 & 52.1 & 63.2 &81.9& 85.8&85.6&76.6  \\
 
\midrule 
\datasetcell{ HumanEval}{0-Shot}{\cite{chen2021evaluating} }       & 74.4 & 37.8 & 39.6 & 62.2&61.0 & 28.0 & 34.1 & 60.4 &78.7& 62.2&92.1&64.4 \\[1.5ex]
\datasetcell{ MBPP}{3-Shot}{\cite{austin2021program} }             & 80.3 & 60.2 & 70.7 & 75.2&71.7 & 50.8 & 51.5 & 67.7 &81.3& 77.8&90.4&77.5  \\
\midrule 
% {\large Average} & 78.55 & 66.70 & 74.48 & 76.85 & 73.69 & 58.92 & 59.22 & 67.34 & 81.2 & 73.78 & 84.76 \\
{\large Average} & 79.58 & 69.62 & 76.20 & 78.46 & 75.74 & 61.23 & 61.73 & 69.40 & 82.78 & 75.27 & 85.70
\end{tabular}
}
\label{table:bbeval}
\end{table}


==> table/gaokao24/13_p.tex <==

\begin{longtable}{ p{.4\textwidth} | p{.6\textwidth} }

\toprule
Question 13 (Correct Answer: $\ln 2$) & Output 13 \\
\midrule
{
\begin{lstlisting}[mathescape,
basicstyle=\small\ttfamily,
columns=flexible,
breaklines=true,
escapeinside={\%*}{*)},
]
If the tangent line to the curve $y = e^x + x$ at the point $(0, 1)$ is also the tangent line to the curve $y = \ln(x+1) + a$, find the value of the constant $a$.

%* 
\color{red}{Note that the curve $y = \ln(x+1) + a$ may or may not pass through the point $(0, 1)$.}
*)
\end{lstlisting}
}  & 
{
\begin{lstlisting}[mathescape,
basicstyle=\small\ttfamily,
columns=flexible,
breaklines=true,
escapeinside={\%*}{*)},
]

First, we find the derivative of $y=e^x+x$ to get the slope of the tangent line at the point $(0,1)$ is $e^0 + 1=2$. 

Next, we find the equation of the tangent line to the curve   $y=\ln(x+1)+a$ at the point $(0, 1)$. Using the point slope form, the equation of the tangent line is $y-1=2(x-0)$, or $y=2x+1$.

Since this tangent line is also the tangent line to the curve $y=ln(x+1)+a$,
the slope of the tangent line to $y=\ln(x+1)+a$ at the point $(0,1)$ must also be 2.

To find the slope of the tangent line to $y=\ln(x+1)+a$ at the point $(0,1)$, we find the derivative of $y=\ln(x+1)+a$ to get $y'=\frac{1}{x+1}$. 


Setting $y′=2$, we have $\frac{1}{x+1}=2$.
Solving for $x$, we find $x=\frac{1}{2}$.

Substituting $x=\frac{1}{2}$ into $y=\ln(x+1) + a$, we have $1=\ln(\frac{1}{2} + 1) + a$. 

Simplifying, we get $1 = \ln(\frac{3}{2}) + a$. 

Finally, we solve for $a$ to find $a=1-\ln(\frac{3}{2})$. 

Therefore, the value of the constant $a$ is $1-\ln(\frac{3}{2})$. The answer is $1-\ln(\frac{3}{2})$.
\end{lstlisting}
} \\

\bottomrule
\end{longtable}


==> table/gaokao24/13_pp_llama3_70b.tex <==

\begin{longtable}{ p{.4\textwidth} | p{.6\textwidth} }

\toprule
Question 13 (Correct Answer: $\ln 2$) & Llama3 70B Output 13 \\
\midrule
{
\begin{lstlisting}[mathescape,
basicstyle=\small\ttfamily,
columns=flexible,
breaklines=true,
escapeinside={\%*}{*)},
]
If the tangent line to the curve $y = e^x + x$ at the point $(0, 1)$ is also the tangent line to the curve $y = \ln(x+1) + a$ %*\color{red}{at some point}*), find the value of the constant $a$
\end{lstlisting}
}  & 
{
\begin{lstlisting}[mathescape,
basicstyle=\scriptsize\ttfamily,
columns=flexible,
breaklines=true,
escapeinside={\%*}{*)},
]
The slope of the tangent line to the curve $y=e^x+x$ at the point $(0,1)$ is $e^0+1=2$. The slope of the tangent line to the curve $y=\ln(x+1)+a$ at the point $(x_0,\ln(x_0+1)+a)$ is $\frac{1}{x_0+1}$. Since these two slopes are equal, we have
$\frac{1}{x_0+1}=2\Rightarrow x_0=\frac{1}{2}$.
Substituting this value into the equation $y=\ln(x+1)+a$, we have
$\ln\left(\frac{3}{2}\right)+a=1\Rightarrow a=1-\ln\left(\frac{3}{2}\right)=\boxed{1-\ln\left(\frac{3}{2}\right)}.$
Final Answer: The final answer is $1-\ln\left(\frac{3}{2}\right)$. I hope it is correct.
\end{lstlisting}
} \\

\bottomrule
\end{longtable}


==> table/gaokao24/6_p.tex <==

\begin{longtable}{ p{.4\textwidth} | p{.6\textwidth} }

\toprule
Question 6 (Correct Answer: B) & Output 6 \\
\midrule
{
\begin{lstlisting}[mathescape,
basicstyle=\small\ttfamily,
columns=flexible,
breaklines=true,
escapeinside={\%*}{*)},
]
Please complete the following single-choice question. The question has four options, and only one of them is correct. Select the option that is correct. 

Question: Given the function 
$$
f(x) = \begin{cases} 
-x^2 - 2ax - a, & x < 0 \\ 
e^x + \ln(x+1), & x \geq 0 
\end{cases}
$$
to ensure $f(x) is strictly increasing on $R$, %*the range of $a$ is\color{red}{:}*)

Option A: $(-\infty, 0]$
Option B: $[-1, 0]$
Option C: $[-1, 1]$
Option D: $[0, \infty)$
\end{lstlisting}
}  & 
{
\begin{lstlisting}[mathescape,
basicstyle=\small\ttfamily,
columns=flexible,
breaklines=true,
escapeinside={\%*}{*)},
]
To ensure that the function $f(x)$ is strictly increasing on R, we need to check the conditions for both parts of the piecewise function.

For x < 0, we have $f(x)=-x^2-2ax-a$. To ensure that this part is strictly increasing, we need to find the range of $a$ such that the derivative of this part is positive.

$f'(x)=-2x-2a$

For $f'(x)$ to be positive, we need -2x - 2a > 0. Since $x < 0$, we have $-2x > 0$. THus, we need $-2a > 0$, which implies $a < 0$.

For $x \geq 0$, we have $f(x)=e^x+ln(x+1)$. The derivative of this part is:

$f'(x)= e^x+\frac{1}{x+1}$

Since $e^x>0$ and $\frac{1}{x+1} > 0$ for $x \geq 0$, we have  $f'(x)>0$ for all $x \geq 0$. 

%*\color{red}{Now, we need to find the range of $a$ such that the functioin is continuous and differentiable at $x=0$.}*) 

For continuity at $x=0$, we need:

$\lim_{x\to0^-}f(x) = \lim_{x\to0^+}f(x)$

$-a = 1 + 0$

$a = -1$

For differentiability at $x=0$, we need:

$\lim_{x\to0^-}f'(x) = \lim_{x\to0^+}f'(x)$

$-2a = 1 + 1$

$a = -1$

Thus, the range of $a$ is $[-1, 0]$. The correct option is $B$: $[-1, 0]$. 
\end{lstlisting}
}  \\
\bottomrule
\end{longtable}


==> table/gaokao24_phi/6_p.tex <==

\begin{longtable}{ p{.4\textwidth} | p{.6\textwidth} }

\toprule
Question 6 (Correct Answer: B) & Output 6 \\
\midrule
{
\begin{lstlisting}[mathescape,
basicstyle=\small\ttfamily,
columns=flexible,
breaklines=true,
escapeinside={\%*}{*)},
]
Please complete the following single-choice question. The question has four options, and only one of them is correct. Select the option that is correct. 

Question: Given the function 
$$
f(x) = \begin{cases} 
-x^2 - 2ax - a, & x < 0 \\ 
e^x + \ln(x+1), & x \geq 0 
\end{cases}
$$
to ensure $f(x) is strictly increasing on $R$, %*the range of $a$ is\color{red}{:}*)

Option A: $(-\infty, 0]$
Option B: $[-1, 0]$
Option C: $[-1, 1]$
Option D: $[0, \infty)$
\end{lstlisting}
}  & 
{
\begin{lstlisting}[mathescape,
basicstyle=\small\ttfamily,
columns=flexible,
breaklines=true,
escapeinside={\%*}{*)},
]
To ensure that the function $f(x)$ is strictly increasing on R, we need to check the conditions for both parts of the piecewise function.

For x < 0, we have $f(x)=-x^2-2ax-a$. To ensure that this part is strictly increasing, we need to find the range of $a$ such that the derivative of this part is positive.

$f'(x)=-2x-2a$

For $f'(x)$ to be positive, we need -2x - 2a > 0. Since $x < 0$, we have $-2x > 0$. THus, we need $-2a > 0$, which implies $a < 0$.

For $x \geq 0$, we have $f(x)=e^x+ln(x+1)$. The derivative of this part is:

$f'(x)= e^x+\frac{1}{x+1}$

Since $e^x>0$ and $\frac{1}{x+1} > 0$ for $x \geq 0$, we have  $f'(x)>0$ for all $x \geq 0$. 

%*\color{red}{Now, we need to find the range of $a$ such that the functioin is continuous and differentiable at $x=0$.}*) 

For continuity at $x=0$, we need:

$\lim_{x\to0^-}f(x) = \lim_{x\to0^+}f(x)$

$-a = 1 + 0$

$a = -1$

For differentiability at $x=0$, we need:

$\lim_{x\to0^-}f'(x) = \lim_{x\to0^+}f'(x)$

$-2a = 1 + 1$

$a = -1$

Thus, the range of $a$ is $[-1, 0]$. The correct option is $B$: $[-1, 0]$. 
\end{lstlisting}
}  \\
\bottomrule
\end{longtable}

